Effect of Nonlinear Surface Inflows into Activity Belts on Solar Cycle Modulation

Converging flows are visible around bipolar magnetic regions (BMRs) on the solar surface, according to observations. Average flows are created by these inflows combined, and the strength of these flows depends on the amount of flux present during the solar cycle. In models of the solar cycle, this average flow can be depicted as perturbations to the meridional flow. In this article, we study the effects of introducing surface inflow to the surface flux transport models (SFT) as a possible nonlinear mechanism in the presence of latitude quenching for an inflow profile whose amplitude varies within a cycle depending on the magnetic activity. The results show that including surface inflows in the model in the presence of both LQ and tilt quenching (TQ) produced a polar field within a $\pm$1$\sigma$ of an average cycle polar field ($\sigma$ is the standard deviation) and a correlation coefficient of 0.85. We confirm that including inflows produces a lower net contribution to the dipole moment (10\,--\,25\%). Furthermore, the relative importance of LQ vs. inflows is inversely correlated with the dynamo effectivity range ($\lambda_{R}$). With no decay term, introducing inflows into the model resulted in a less significant net contribution to the dipole moment. Including inflows in the SFT model shows a possible nonlinear relationship between the surface inflows and the solar dipole moment, suggesting a potential nonlinear mechanism contributing to the saturation of the global dynamo. For lower $\lambda_R$ ($\lessapprox$ 10 $^\circ$), TQ always dominates LQ, and for higher $\lambda_R$ LQ dominate. However, including inflows will make the domination a little bit earlier in case of having a decay term in the model.

==> name.tex <==

\begin{table}
\caption{Set of parameters considered for {inflows whose amplitudes are fixed in every cycle} from profile (I) and its deviations of the nonlinear models $|\Delta D_n|$ from the linear case measured at a certain SSN value.}
\label{table:dev_inflow}
\begin{tabular}{lllllll}    
\hline  \\  
	Case & $u_{0}$ & $\eta$ & $\tau$ &  $dev$ & $\devLQ$ &  $dev$\\
  &[m$/$s]  & [km$^2/$s] & [yr] & \tiny LQ+inflows& & \tiny inflows  \\
\\
\hline
 a & 11 &250 & 8 & 2.098 & 1.600 & 0.373\\
 b & 11 &350 & 8 & 1.832 & 1.455 & 0.366 \\
 c & 11 &450 & 8 & 1.582 & 1.185 & 0.277\\
 d & 11 &600 & 8 & 1.074 & 0.734 & 0.249\\
 e & 11 &250 & $\infty$ & 1.750 & 1.407 & 0.493 \\
 f & 11 &350 & $\infty$ & 1.659 & 1.249 & 0.436 \\
 g & 11 &450 & $\infty$ & 1.439 & 0.998 & 0.468\\
 h & 11 &600 & $\infty$ & 1.164 & 0.768 & 0.432\\
\hline
\end{tabular}
\end{table}




\begin{figure}    %%%%%%%%%%%%%%%%%% FIGURE 2 
\centerline{\includegraphics[width=0.5\textwidth,clip=]{Jiang_quad_u.png}}
\small
        \caption{Relative importance of LQ vs. inflows plotted against the $u_{0}/\eta$ ratio. Separate quadratic fits for the case $\tau = 8$ (blue) and $\tau = \infty$ (orange) are shown for the different parameter combinations listed in Table~\ref{table:dev_inflow} for the inflow profile (I).}
\label{fig:inflow}
\end{figure}


\begin{table*}[t]
\caption{Fitting parameters of $|\Delta D(t)|$ vs. $S_{max},n$ for inflows, LQ, and LQ+inflows cases using profile (I) following a quadratic polynomial of the form $c_1x^2+c_2x+c_3$.}
\label{table:fit_parm1}
\begin{tabular}{@{}cccccccccc@{}}    
\hline  \\  
	Case &  \multicolumn{3}{c}{inflows} &  \multicolumn{3}{c}{LQ} &   \multicolumn{3}{c}{LQ+inflows}\\\hline
 & $c_{1}\times 10^{-6}$ &$c_{2}$ &$c_{3}$ &$c_{1}\times 10^{-5}$ &$c_{2}$ &$c_{3}$ &$c_{1}\times 10^{-5}$ &$c_{2}$ &$c_{3}$ \\
\hline
a&5.11&0.028&-0.001&-4.17&0.038&-0.059&-3.41&0.034&0.001\\
b&5.20&0.031&-0.012&-3.69&0.040&-0.147&-3.18&0.037&-0.135\\
c&4.66&0.033&-0.019&-3.16&0.041&-0.204&-2.63&0.039&-0.169\\
d&4.02&0.034&-0.022&-2.36&0.041&-0.247&-1.87&0.039&-0.200\\
e&1.31&0.023&-0.019&-3.32&0.030&0.028&-3.10&0.028&-0.003\\
f&1.56&0.025&-0.031&-3.18&0.033&-0.111&-2.85&0.030&-0.076\\
g&1.44&0.027&-0.038&-2.76&0.034&-0.157&-2.57&0.032&-0.147\\
h&1.37&0.028&-0.031&-2.18&0.035&-0.208&-2.06&0.033&-0.201\\
\hline
\end{tabular}
\end{table*}


\begin{figure}    %%%%%%%%%%%%%%%%%% FIGURE 3 
\centerline{\includegraphics[width=0.5\textwidth,clip=]{lambdaR_invx8.png}}
\small
        \caption{The relative importance of LQ vs. inflows is plotted against the dynamo effectivity range, $\lambda_R$, for the parameter combinations listed in Table~\ref{table:dev_inflow}. Distinct fit to Eq.~(\ref{eq:fit2}) are shown for $\tau=8$ (blue), and $\tau=\infty$ (orange) for $n = 2$.}
\label{fig:lambda_r_J}
\end{figure}

\begin{figure}    %%%%%%%%%%%%%%%%%% FIGURE 1 
\centerline{\includegraphics[width=0.5\textwidth,clip=]{case11_250_1000.png}}
\small
        \caption{Net contribution of a cycle to the solar dipolar moment vs. cycle amplitude for the different cases with respect to the linear case with no quenching. The parameter values were $u_0=11\,$m$/$s, $\eta=250\,$km$^2/$s and $\tau = \infty $ years. inflows are implemented with an amplitude $v_0=5$ m$/$s for {inflows whose amplitudes are fixed in every cycle} introduced by \citet{jiang2010effect}. The dashed and solid vertical lines show the average and twice average cycle amplitude values respectively, the horizontal dashed lines show where the twice average vertical line intersects with each case.}
\label{fig:quad_fit}
\end{figure}
\begin{table*}[t]
\caption{Fitting parameters of $|\Delta D(t)|$ vs. $S_{max},n$ for inflows, LQ and LQ+inflows cases using profile (II) following a quadratic polynomial of the form $c_1x^2+c_2x+c_3$.}
\label{table:fit_parm}
\begin{tabular}{@{}cccccccccc@{}}    
\hline  \\  
	Case &  \multicolumn{3}{c}{inflows} &  \multicolumn{3}{c}{LQ} &   \multicolumn{3}{c}{LQ+inflows}\\\hline
 & $c_{1}\times 10^{-6}$ &$c_{2}$ &$c_{3}$ &$c_{1} \times 10^{-5}$ &$c_{2}$ &$c_{3}$ &$c_{1}\times 10^{-5}$ &$c_{2}$ &$c_{3}$ \\
\hline
a&6.896&0.027&0.017&-4.175&0.038&-0.062&-3.381&0.033&-0.045\\
b&7.470&0.030&0.005&-3.680&0.040&-0.146&-2.878&0.035&-0.107\\
c&7.026&0.032&-0.007&-3.135&0.041&-0.198&-2.407&0.037&-0.158\\
d&6.479&0.033&-0.013&-2.593&0.041&-0.225&-2.150&0.038&-0.245\\
e&6.246&0.033&-0.010&-2.407&0.042&-0.258&-1.764&0.038&-0.213\\
f&1.668&0.022&-0.011&-3.424&0.030&-0.006&-2.906&0.026&0.024\\
g&2.011&0.024&-0.028&-3.176&0.033&-0.108&-2.736&0.029&-0.070\\
h&2.054&0.026&-0.032&-2.817&0.034&-0.173&-2.414&0.030&-0.120\\
i&1.939&0.027&-0.034&-2.385&0.035&-0.201&-2.063&0.031&-0.151\\
j&1.898&0.028&-0.033&-2.093&0.034&-0.186&-1.920&0.031&-0.173\\
k&9.213&0.025&0.068&-4.175&0.038&-0.062&-3.107&0.032&-0.015\\
l&0.1004&0.028&0.036&-3.680&0.040&-0.146&-2.594&0.034&-0.084\\
m&0.1048&0.030&0.037&-3.135&0.041&-0.198&-2.114&0.036&-0.131\\
n&9.034&0.031&0.003&-2.593&0.041&-0.225&-1.706&0.036&-0.175\\
o&8.717&0.032&0.003&-2.407&0.042&-0.258&-1.457&0.036&-0.174\\
p&1.701&0.021&0.005&-3.424&0.030&-0.006&-2.849&0.026&0.019\\
q&2.395&0.023&-0.018&-3.176&0.033&-0.108&-2.595&0.028&-0.054\\
r&2.661&0.025&-0.024&-2.817&0.034&-0.173&-2.337&0.030&-0.120\\
s&2.485&0.026&-0.033&-2.385&0.035&-0.201&-1.990&0.030&-0.147\\
t&2.657&0.026&-0.023&-2.093&0.034&-0.186&-1.833&0.031&-0.161\\
\hline
\end{tabular}
\end{table*}
